Injecting Imbalance Sensitivity for Multi-Task Learning

Multi-task learning (MTL) has emerged as a promising approach for deploying deep learning models in real-life applications. Recent studies have proposed optimization-based learning paradigms to establish task-shared representations in MTL. However, our paper empirically argues that these studies, specifically gradient-based ones, primarily emphasize the conflict issue while neglecting the potentially more significant impact of imbalance/dominance in MTL. In line with this perspective, we enhance the existing baseline method by injecting imbalance-sensitivity through the imposition of constraints on the projected norms. To demonstrate the effectiveness of our proposed IMbalance-sensitive Gradient (IMGrad) descent method, we evaluate it on multiple mainstream MTL benchmarks, encompassing supervised learning tasks as well as reinforcement learning. The experimental results consistently demonstrate competitive performance.

==> sec/discussion.tex <==
\section{Discussion with Counterparts}
To the best of our knowledge, IMTL~\cite{liutowards} and NashMTL~\cite{navon2022multi} are two recent works that consider imbalance issue as well. However, both two works fail to provide evidence to show the importance of imbalance issue. Neither do they own conflict-averse property. Thus, they still have the room for improvements. As for NashMTL, although its design seems to be conflict-averse, its practical implementation fails to achieve it. Please refer to the \textbf{Appendix} for more details.
